Classifying Eyes-Free Mobile Authentication Techniques

Mobile device users avoiding observational attacks and coping with situational impairments may employ techniques for eyes-free mobile unlock authentication, where a user enters his/her passcode without looking at the device. This study supplies an initial description of user accu- racy in performing this authentication behavior with PIN and pattern passcodes, with varying lengths and visual characteristics. Additionally, we inquire if tactile-only feedback can provide assistive spatialization, finding that orientation cues prior to unlocking do not help. Measure- ments of edit distance and dynamic time warping accuracy were collected, using a within-group, randomized study of 26 participants. 1,021 passcode entry gestures were collected and classified, identifying six user strategies for using the pre-entry tactile feedback, and ten codes for types of events and errors that occurred during entry. We found that users who focused on orienting themselves to position the first digit of the passcode using the tactile feedback performed better in the task. These results could be applied to better define eyes-free behavior in further research, and to design better and more secure methods for eyes-free authentication.

==> whatsnew.tex <==
\section{What's New}
\todo{It may be a good idea to remove the What's New section, as this has already been seen by reviewers.  We can also do this if this version is accepted.}
The research described in the manuscript for submission to JISA relates to a study examining user accuracy when authenticating under eyes-free settings.  More specifically, the study provides an insight into the ways in which PIN and pattern selection (i.e., varying lengths and spatial characteristics) may impact accurate entry, and whether tactile-only feedback can support the spatialization process.  

A shorter paper based on our initial work was accepted by the Workshop on Usable Security (USEC 2018) in the work-in progress track (entitled “Work-In-Progress: Performance of Eyes-Free Mobile Authentication”).  The paper provided a general overview of our study, along with preliminary analysis.  However, we have added additional content to all sections, and vastly extended the analysis focusing on classification techniques.  The three research questions described in the manuscript submitted to JISA have been addressed in significant detail, in contrast to our prior paper.

In the manuscript submitted to JISA, we have described the use of Dynamic Time Warping techniques to identify precision of the user, the ways in which edit distance measurements have been calculated, and our process and metrics used to classify interaction behaviors.  Six training classifications and ten entry classifications have been identified, which can be used by other researchers aiming to classify their own traces.  Findings from the qualitative analysis of our data has also been added to the manuscript to supplement the quantitative analysis presented. 

In contrast to the contributions outlined in our earlier publication, the additional analysis submitted to JISA has shown:
\begin{enumerate}
  \item We have demonstrated the extension of existing classification methodology for coding eyes-free unlock entry methods and events, similar to error codes established in von Zezschwitz et al. \cite{von2013patterns}.  
\item We have identified significant relationships between classification codes and authentication conditions (e.g. a decrease in Start-Hunt behavior for pattern passcodes ($\chi^2=8.17, p<0.005$).
\item  We have identified passcodes features for which accuracy and/or precision significantly deviated from average (e.g. self-crossing pattern 743521).
 \end{enumerate}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

